Parallel line segments

In this article I will address some questions about a mathematical problem that my friend Patrizio Frederic, a researcher in statistics at the University of Modena, proposed to me. Given some parallel line segments, is there at least one straight line that passes through all of them? If there were many lines that solve the problem, can I choose a "best one" among all of them? I will fully address the first question. As for the second question, I will illustrate it with some "experimental" examples and suggest an outline for future explorations.

==> pst-vect.tex <==
%%%
%%% BEGIN: pst-vect.tex
%%%
\def\fileversion{2.2}
\def\filedate{2007/07/07}
%%%
\csname PSTvectLoaded\endcsname
\let\PSTvectLoaded\endinput
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi\relax
\ifx\PSTthreeDLoaded\endinput\else\input pst-3d.tex\fi\relax
\RequirePackage{pst-pic}
\pstheader{pst-vect.pro}
%%%--------------------------------------------------------------------------------------------------------------------------------------
\makeatletter
%%%===================================================================================
\begingroup
\catcode`\|=13
\catcode`\;=13
\catcode`\+=13
\catcode`\*=13
\catcode`\?=13
\catcode`\>=13
\catcode`\<=13
\catcode`\!=13
\catcode`\/=13
\catcode`\`=13
\gdef\pst@activemathcoor{%
  \def|{\string|}%
  \def;{\string;}%
  \def+{\string+}%
  \def*{\string*}%
  \def?{\string?}%
  \def>{\string>}%
  \def<{\string<}%
  \def!{\string!}%
  \def/{\string/}%
  \def`{\string`}}
\endgroup
%%%===================================================================================
\def\MathCoor{%
  \SpecialCoor
  \def\pst@@getcoor##1{%
    \begingroup
    \pst@activemathcoor
    \xdef\pst@tempg{##1}%
    \endgroup
    \expandafter\if@sum@coor\pst@tempg+;\@nil}}
%%%===================================================================================
\def\if@sum@coor#1+{%
  \@ifnextchar;{\if@mul@coor#1*}{\sum@coor#1+}}
\def\sum@coor#1+#2\@nil{%
  \begingroup
  \if@sum@coor#2\@nil
  \let\pst@sumx\pst@coor
  \if@mul@coor#1*;\@nil
  \xdef\pst@tempg{\pst@sumx exch \pst@coor 3 1 roll add 3 1 roll add }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\if@mul@coor#1*{%
  \@ifnextchar;{\if@rotate@coor#1?}{\@mul@coor{#1}}}
\def\@mul@coor#1#2*;\@nil{%
  \begingroup
  \isit@modulo@coor#1]\@nil
  \if@sum@coor#2+;\@nil
  \xdef\pst@tempg{\pst@coor \vect@number dup 4 3 roll mul 3 1 roll mul }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\if@rotate@coor#1?{%
  \@ifnextchar;{\if@vect@coor#1>}{\rotate@coor{#1}}}
\def\rotate@coor#1#2?;\@nil{%
  \begingroup
  \isit@angle@coor#1]\@nil
  \if@sum@coor#2+;\@nil
  \xdef\pst@tempg{%
    \pst@coor \vect@number dup sin exch cos 4 copy 4 3 roll mul 
    3 1 roll mul sub 5 1 roll 3 2 roll mul 3 1 roll mul add }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\isit@modulo@coor{%
  \@ifnextchar`{\modulo@coor}{\number@coor}}
\def\isit@angle@coor{%
  \@ifnextchar`{\angle@coor}{\number@coor}}
\def\angle@coor`{\@ifnextchar`{\angle@neg@coor}{\angle@@coor}}
\def\angle@neg@coor`#1]\@nil{%
  \if@sum@coor#1+;\@nil
  \edef\vect@number{\pst@coor exch 2 copy dup 
    mul exch dup mul add 0 eq {pop} {atan} ifelse neg }}
\def\angle@@coor#1]\@nil{%
  \if@sum@coor#1+;\@nil
  \edef\vect@number{\pst@coor exch 2 copy dup 
    mul exch dup mul add 0 eq {pop} {atan} ifelse }}
\def\modulo@coor`{\@ifnextchar`{\modulo@div@coor}{\modulo@@coor}}
\def\modulo@div@coor`#1]\@nil{%
  \if@sum@coor#1+;\@nil
  \edef\vect@number{1 \pst@coor \back@unit dup 
    mul exch dup mul add sqrt dup 0 eq {pop} {div} ifelse }}
\def\modulo@@coor#1]\@nil{%
  \if@sum@coor#1+;\@nil
  \edef\vect@number{\pst@coor \back@unit dup mul exch dup mul add sqrt }}
\def\number@coor#1]\@nil{%
  \edef\vect@number{#1 }}
%%%===================================================================================
\def\if@vect@coor#1>{%
  \@ifnextchar;{\if@mixed@coor#1|}{\vect@coor{#1}}}
\def\vect@coor#1#2>;\@nil{%
  \begingroup
  \if@sum@coor#2+;\@nil
  \let\pst@vectx\pst@coor
  \if@sum@coor#1+;\@nil
  \xdef\pst@tempg{\pst@vectx exch \pst@coor 3 1 roll sub 3 1 roll sub }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\if@mixed@coor#1|{%
  \@ifnextchar;{\if@versus@coor#1;}{\math@mixed@coor{#1}}}
\def\math@mixed@coor#1#2|;\@nil{%
  \begingroup
  \if@sum@coor#1+;\@nil
  \let\pst@tempa\pst@coor
  \if@sum@coor#2+;\@nil
  \xdef\pst@tempg{\pst@tempa pop \pst@coor exch pop }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\if@versus@coor{%
  \@ifnextchar/{\versus@coor}{\if@raw@coor}}
\def\versus@coor/#1;;\@nil{%
  \begingroup
  \if@sum@coor#1+;\@nil
  \xdef\pst@tempg{\pst@coor exch 2 copy dup mul exch dup mul 
    add dup 0 eq {pop 1} if sqrt dup 3 1 roll div 3 1 roll div \step@unit }%
  \endgroup
  \let\pst@coor\pst@tempg}
%%%===================================================================================
\def\if@raw@coor{%
  \@ifnextchar!{\math@raw@coor}{\if@polar@coor}}
\def\math@raw@coor!#1;;\@nil{%
  \edef\pst@coor{#1 \step@unit }}
%%%===================================================================================
\def\if@polar@coor#1;{%
  \@ifnextchar;{\if@cartesian@coor#1,}{\math@polar@coor{#1}}}
\def\math@polar@coor#1#2;;\@nil{%
  \edef\pst@coor{#2 cos #1 mul #2 sin #1 mul \step@unit }}
%%%===================================================================================
\def\if@cartesian@coor#1,{%
  \@ifnextchar;{\isit@vector@coor#1;}{\math@cartesian@coor{#1}}}
\def\math@cartesian@coor#1#2,;\@nil{%
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}}%
%%%===================================================================================
\def\isit@vector@coor{%
  \@ifnextchar<{\what@node@coor}{\vector@coor}}
\def\what@node@coor<{%
  \@ifnextchar[{\Node@coor}{\node@coor}}
\def\vector@coor#1;;\@nil{%
  \edef\pst@coor{V@#1 \step@unit }}
%%%===================================================================================
\def\vnode{\@ifnextchar({\vnode@}{\vnode@(0,0)}}
\def\vnode@(#1)#2{%
  \pst@getvect{#1}\pst@vecta%
  \pnode@(!/V@#2 {\pst@vecta} bind def V@#2){#2}}
%%%===================================================================================
\def\back@unit{\pst@number\psyunit div exch \pst@number\psxunit div exch }
\def\step@unit{\pst@number\psyunit mul exch \pst@number\psxunit mul exch }
\def\pst@getvect#1#2{%
  \begingroup
  \pst@@getcoor{#1}%
  \xdef\pst@tempg{\pst@coor \back@unit }%
  \endgroup
  \let#2\pst@tempg}
%%%===================================================================================
%%%===================================================================================
%%%===================================================================================
\def\intersection(#1)(#2)(#3){\@ifnextchar({\@inters(#1)(#2)(#3)}{\@inters(0,0)(#1)(#2)(#3)}}
\def\@inters(#1)(#2)(#3)(#4)#5{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \pst@getvect{#4}\pst@vectd%
  \vnode(!\pst@vecta \pst@vectb \pst@vectc \pst@vectd inters){#5}}
%%%===================================================================================
\def\projection(#1)(#2){\@ifnextchar({\@projec(#1)(#2)}{\@projec(0,0)(#1)(#2)}}
\def\@projec(#1)(#2)(#3)#4{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \vnode(!\pst@vecta \pst@vectb \pst@vectc proiez){#4}}
%%%===================================================================================
\def\axesxy#1(#2)(#3){\@ifnextchar({\axesxy@#1(#2)(#3)}{\axesxy@#1(0,0)(#2)(#3)}}
\def\axesxy@#1(#2)(#3)(#4){\axes#1(#2)(#3)(#4){$x$}{$y$}}
\def\axesreim#1(#2)(#3){\@ifnextchar({\axesreim@#1(#2)(#3)}{\axesreim@#1(0,0)(#2)(#3)}}
\def\axesreim@#1(#2)(#3)(#4){\axes#1(#2)(#3)(#4){Re}{Im}}
\def\axes{\@ifnextchar[{\axes@}{\axes@[fillstyle=none]}}
\def\axes@#1(#2)(#3){\@ifnextchar({\axes@@#1(#2)(#3)}{\axes@@#1(0,0)(#2)(#3)}}
\def\axes@@[#1](#2)(#3)(#4)#5#6{{\psset{#1}%
  \psline{->}({#3}|{#2})({#4}|{#2})
  \psline{->}({#2}|{#3})({#2}|{#4})
  \uput{2pt}[270]({#4}|{#2}){#5}
  \uput{2pt}[0]({#2}|{#4}){#6}}}
%%%===================================================================================
\def\mediumpoint(#1){%
  \@ifnextchar({\medium@point(#1)}{\medium@point(0,0)(#1)}}
\def\medium@point(#1)(#2)#3{%
  \vnode(0.5*{{#1}+{#2}}){#3}}
%%%===================================================================================
\def\incenter(#1)(#2)(#3)#4{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \vnode(!\pst@vecta \pst@vectb \pst@vectc incentro){#4}}
%%%===================================================================================
\def\barycenter{\centroid}
\def\centroid(#1)(#2)(#3)#4{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \vnode(!\pst@vecta exch \pst@vectb \pst@vectc exch 
  5 3 roll add add 3 div 4 1 roll add add 3 div){#4}}
%%%===================================================================================
\def\orthocenter(#1)(#2)(#3)#4{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \vnode(!\pst@vecta  \pst@vectb  \pst@vectc  ortoc){#4}}
%%%===================================================================================
\def\circumcenter(#1)(#2)(#3)#4{%
  \pst@getvect{#1}\pst@vecta%
  \pst@getvect{#2}\pst@vectb%
  \pst@getvect{#3}\pst@vectc%
  \vnode(!\pst@vecta \pst@vectb \pst@vectc circoc){#4}}
%%%===================================================================================
\def\circleCP{\@ifnextchar[{\circle@CP,}{\circle@CP[]}}
\def\circle@CP#1[#2](#3)(#4){%
  \psellipse[showpoints=false#1#2](#3)(`{#3}>{#4}*{1,1})}
%%%===================================================================================
\def\rightangle{\@ifnextchar[{\right@angle,}{\right@angle[]}}
\def\right@angle#1[#2](#3)(#4){\@ifnextchar({\right@@angle[#1#2](#3)(#4)}{\right@@angle[#1#2](#3)(0,0)(#4)}}
\def\right@@angle[#1](#2)(#3)(#4){%
  \rput(#3){\psset{unit=2.5mm,dotstyle=*,linewidth=.3pt,showpoints=false,dotsize=2pt#1}%
    \psline(/{{#3}>{#2}})(/{{#3}>{#2}}+/{{#3}>{#4}})(/{{#3}>{#4}})
    \psdots(0.5*{/{{#3}>{#2}}+/{{#3}>{#4}}})}}
%%%===================================================================================
\def\arcangle{\@ifnextchar[{%
    \arcangle@i,}{%
    \arcangle@i[]}}
\def\arcangle@i#1[#2]{\@ifnextchar({%
    \arcangle@ii[#1#2]8mm}{%
    \arcangle@ii[#1#2]}}
\def\arcangle@ii#1(#2)#3(#4)(#5){%
  \ifx#3`\arcangle@iii#1(#5)(#4)(#2)
  \else\arcangle@iii#1(#2)(#4)(#5)\fi}
\def\arcangle@iii[#1]#2(#3)(#4)(#5){%
  \psarc[linewidth=.3pt#1](#4){#2}{({#4}>{#3})}{({#4}>{#5})}}
%%%===================================================================================
\def\labelangle{\@ifnextchar*{%
    \def\rp@t{\rput*}\labelangle@i}{%
    \def\rp@t{\rput}\labelangle@i*}}
\def\labelangle@i*{\@ifnextchar[{%
    \labelangle@ii}{%
    \labelangle@iii{}}}
\def\labelangle@ii[#1]{\labelangle@iii{[#1]}}
\def\labelangle@iii#1#2(#3)#4(#5)(#6)#7{%
  \ifx#4`\labelangle@iv#2///(#6)(#5)(#3){#7}{#1}
  \else\labelangle@iv#2///(#3)(#5)(#6){#7}{#1}\fi}
\def\labelangle@iv{\@ifnextchar/{%
    \labelangle@v8mm}{%
    \labelangle@v}}
\def\labelangle@v#1/{\@ifnextchar/{%
    \labelangle@vi#1/0.7}{%
   \labelangle@vi#1/}}
\def\labelangle@vi#1/#2/{\@ifnextchar/{%
    \labelangle@vii#1/#2/0.5}{%
    \labelangle@vii#1/#2/}}
\def\labelangle@vii#1/#2/#3/#4(#5)(#6)(#7)#8#9{%
  \pst@getvect{#5}\pst@vecta%
  \pst@getvect{#6}\pst@vectb%
  \pst@getvect{#7}\pst@vectc%
  \pssetlength\pst@dimg{#1}%
  \def\x@dim{#2 \pst@number\pst@dimg \pst@number\psxunit div mul mul }%
  \def\y@dim{#2 \pst@number\pst@dimg \pst@number\psyunit div mul mul }%
  \rp@t({#6}+!\pst@vecta \pst@vectb \pst@vectc 2ang 2 copy lt {exch 360 add exch} if 
  dup 3 1 roll sub #3 mul add dup cos \x@dim exch sin \y@dim){#8}%
  \arcangle#9#1(#5)(#6)(#7)}
%%%===================================================================================
\def\@ifgrop#1#2{\@ifnextchar`{#1}{\@ifnextchar({#1}{#2}}}
\def\@ifgropoe#1#2{\@ifgrop{#1}{\@ifnextchar>{#1}{#2}}}
%%%===================================================================================
\def\point{\@ifnextchar*{\def\up@t{\uput*}\point@i}{\def\up@t{\uput}\point@i*}}
\def\point@i*{\@ifnextchar[{\point@ii,}{\point@ii[]}}
\def\point@ii#1[#2]{\@ifnextchar({\point@iii[#1#2]2pt}{\point@iii[#1#2]}}
\def\point@iii[#1]#2(#3)#4(#5)(#6)#7{%
  \ifx#4`\point@iii[#1]#2(#6)(#5)(#3){#7}
  \else{\psset{dotstyle=o,dotsize=2.3pt#1}%
  \psdots(#5)\vnode(#3){nnA}\vnode(#5){nnB}\vnode(#6){nnC}%
  \up@t{#2}[!V@nnA V@nnB V@nnC label](#5){#7}}\fi}
%%%===================================================================================
\def\vpoint#1({\vpoint@i#1`(}
\def\vpoint@i#1`#2(#3)#4(#5){%
  \ifx#2`\def\next{\vpoint@ii#1(#5)}%
  \else\def\next{\vpoint@ii#1}\fi%
  \next(#3)#4(#5)}
\def\vpoint@ii#1(#2)#3(#4)#5(#6){\point#1(#2)#3(#4)(#6){$#4$}%
  \@ifgrop{\vpoint@ii#1(#4)#5(#6)}{\ifx#5`\point#1(#4)(#6)(#4){$#6$}\fi}}
%%%===================================================================================
\def\vlines{\@ifnextchar[{\vlines@i{arrows=c-c,linearc=0.1pt,}}{\vlines@i[arrows=c-c,linearc=0.1pt]}}
\def\vlines@i#1[#2]#3(#4){\vlines@ii[#1#2]#3`(#4)}
\def\vlines@ii[#1]#2`#3(#4)#5(#6){%
  \ifx#3`\def\@next{\vlines@iv{[#1](#4)}{[#1]#2(#6)(#4)}}
  \else\def\@next{\vlines@iii[#1]#2<}\fi
  \@next(#4)#5(#6)}
\def\vlines@iii[#1]#2<#3(#4)#5(#6){%
  \ifx#3<\def\@next{\vlines@iv{[#1](#4)}{[#1]#2(#4)}}
  \else\def\@next{\vlines@iv{[#1]}{[#1]#2(#4)}}\fi
  \@next(#4)#5(#6)}
\def\vlines@iv#1#2(#3)#4(#5){\@ifgropoe{%
    \vlines@iv{#1(#5)}{#2#4(#5)}(#5)}{%
    \ifx#4`\psline#1(#5)\vpoint#2(#5)(#3)
    \else\ifx#4>\psline#1(#5)\vpoint#2(#5)
    \else\psline#1\vpoint#2(#5)\fi\fi}}
%%%===================================================================================
%%%===================================================================================
%%%===================================================================================
%%%===================================================================================
%\def\vlines{\@ifnextchar[{\vlines@i{arrows=c-c,}}{\vlines@i[arrows=c-c]}}
%\def\vlines@i#1[#2]#3({\vlines@ii[#1#2]#3`(}
%\def\vlines@ii[#1]#2`#3(#4)#5(#6){%
%  \ifx#3`\def\@next{\vlines@iii{[#1]#2(#6)(#4)}}%
%  \else\def\@next{\vlines@iii{[#1]#2(#4)}}\fi%
%  \@next(#4)#5(#6)}
%\def\vlines@iii#1(#2)#3(#4){\@ifgrop{%
%    \vlines@iii{#1#3(#4)}(#4)}{%
%    \ifx#3`\vlines@iv#1(#4)(#2)%
%    \else\vlines@iv#1(#4)\fi}}
%\def\vlines@iv[#1]#2(#3)#4(#5)#6(#7){\@ifgrop{%
%    \psline[#1](#5)(#7)\point[#1]#2(#3)#4(#5)(#7){$#5$}\vlines@iv[#1]#2(#5)#6(#7)}{%
%    \point[#1]#2(#3)#4(#5)(#7){$#5$}}}
%%%===================================================================================
\def\ABC{\vpolygon(A)(B)(C)}
\def\vpolygon{\@ifnextchar[{\vpolygon@i{linearc=0.2pt,}}{\vpolygon@i[linearc=0.2pt]}}
\def\vpolygon@i#1[#2]#3(#4){\vpolygon@ii[#1#2]#3`(#4)}
\def\vpolygon@ii[#1]#2`#3(#4)#5(#6){\vpolygon@iii{[#1](#4)}{[#1]#2(#4)}{#3(#4)(#6)}#5(#6)}
  \def\vpolygon@iii#1#2#3#4(#5){\@ifgrop{%
      \vpolygon@iii{#1(#5)}{#2#4(#5)}{#3}}{%
      \pspolygon#1(#5)\vpoint#2#4(#5)#3}}
%%%%===================================================================================
%\def\vpoint#1(#2)#3(#4)#5(#6){\point#1(#2)#3(#4)(#6){$#4$}\@ifgrop{\vpoint#1(#4)#5(#6)}{}}
%%%%===================================================================================
%\def\point{\@ifnextchar*{\def\up@t{\uput*}\point@i}{\def\up@t{\uput}\point@i*}}
%\def\point@i*{\@ifnextchar[{\point@ii,}{\point@ii[]}}
%\def\point@ii#1[#2]{\@ifnextchar({\point@iii[#1#2]3pt}{\point@iii[#1#2]}}
%\def\point@iii[#1]#2(#3)#4(#5)(#6)#7{%
%  \ifx#4`\point@iii[#1]#2(#6)(#5)(#3){#7}
%  \else{\psset{dotstyle=o,dotsize=2.3pt#1}%
%  \psdots(#5)\vnode(#3){nnA}\vnode(#5){nnB}\vnode(#6){nnC}%
%  \up@t{#2}[!V@nnA V@nnB V@nnC label](#5){#7}}\fi}
%%%%===================================================================================
%\def\vpolygon{\@ifnextchar[{\vpolygon@i{3pt,}}{\vpolygon@i[3pt]}}
%\def\vpolygon@i#1[#2]{\def\sett@{\sett@@#1#2,,}\@ifgrop{\vpolygon@ii}{\vpolygon@iii{(A)}(A)\@nil(B)(C)}}
%\def\vpolygon@ii#1(#2){\@ifgrop{\vpolygon@iii{}{}\@nil#1(#2)}{\vpolygon@iii{(A)(B)}(A)(B)\@nil(C)#1(#2)}}
%\def\vpolygon@iii#1#2\@nil#3(#4)#5(#6){%
%  \@ifgrop{\vpolygon@iii{#1(#4)}#2#3(#4)\@nil#5(#6)}{\def\vp@int{\vpoint}{%
%    \sett@\pspolygon#1(#4)(#6)\vp@int(#4)#5(#6)#2#3(#4)(#6)}}}
%%%%===================================================================================
%\def\n@n,{}
%\def\sett@@#1,{\sett@@@#1==\@nil\@ifnextchar,{\n@n}{\sett@@}}
%\def\sett@@@#1=#2=#3\@nil{\ifx#3=\psset{#1={#2}}\else\def\vp@int{\vpoint{#1}}\fi}
%%%%===================================================================================
%\def\vlines{\@ifnextchar[{\vlines@i{3pt,}}{\vlines@i[3pt]}}
%\def\vlines@i#1[#2]{\def\sett@{\sett@@#1#2,,}\vlines@ii}
%\def\vlines@ii#1(#2)#3(#4){\ifx#1`\def\U@U{\vlines@iii{(#2)}(#4)}\else\def\U@U{\vlines@iii{}{}}\fi\U@U\@nil(#2)#3(#4)}
%\def\vlines@iii#1#2\@nil(#3)#4(#5){%
%  \@ifgrop{\vlines@iii{#1(#5)}#2(#3)#4\@nil(#5)}{\def\vp@int{\vpoint}{%
%      \sett@\ifx#4`\psline#1(#5)\vpoint#2(#3)(#5)(#3)%
%    \else\psline#1\vpoint#2(#3)(#5)\fi}}}
%%%===================================================================================
\def\lineAB{\@ifnextchar({\lineAB@iv}{\@ifnextchar/{\lineAB@v}{\lineAB@i}}}
\def\lineAB@i#1({\lineAB@ii#1/(}
\def\lineAB@ii#1/{\@ifnextchar({\lineAB@iii#1}{\lineAB@vi#1/}}
\def\lineAB@iii#1(#2)(#3)#4/{\lineAB@vi#1/#4/(#2)(#3)#4/}
\def\lineAB@iv(#1)(#2)#3/#4/{\lineAB@vi#4/#3/(#1)(#2)#3/#4/}
\def\lineAB@v/#1(#2)(#3)#4/#5/{\lineAB@vi#5/#1/(#2)(#3)#4/#5/}
\def\lineAB@vi#1/#2/(#3)(#4)#5/#6/{%
  \psline[linestyle=dashed]({#3}+{#1 #2 add}*{{#4}>{#3}})({#4}+{#5 #6 add}*{{#3}>{#4}})%
  \psline({#3}+#2*{{#4}>{#3}})({#4}+#5*{{#3}>{#4}})}
%%%===================================================================================
\def\name{\@ifnextchar*{\def\up@t{\uput*}\name@}{\def\up@t{\uput}\name@*}}
\def\name@*#1(#2){\@ifnextchar({\name@@#1//(#2)}{\name@@#1//(0,0)(#2)}}
\def\name@@{\@ifnextchar/{\name@@@1.5pt}{\name@@@}}
\def\name@@@#1/{\@ifnextchar/{\name@@@@#1/0.5}{\name@@@@#1/}}
\def\name@@@@#1/#2/#3(#4)(#5)#6{%
  \up@t{#1}[(90?{#5}>{#4})](#2*{{#4}+{#5}}){#6}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\name{\@ifnextchar*{\def\lp@t{\lput*}\name@}{\def\lp@t{\lput}\name@*}}		VECIO
%\def\name@*{\@ifnextchar({\name@@5pt}{\name@@}}
%\def\name@@#1(#2)(#3)#4{\pcline[offset=#1,linestyle=none](#3)(#2)\lp@t{0}{#4}}
%%%===================================================================================
\def\vnodedef#1#2#3{\vnode(!/#1 {#2} bind def 0 0){#3}}
%%%===================================================================================
\def\treD#1#2(#3)#4{%
  \tre@D(#3,){#1}{#2}{#4}}
\def\tre@D(#1,#2,{\@ifnextchar){\tre@@D#1(#2,}{\tre@@D#1,#2(}}
\def\tre@@D#1(#2,)#3#4#5{%
  \pst@getvect{#1}\pst@vecta%
  \vnode(!\pst@vecta exch pop #2+\pst@vecta pop*#4*#3?!1 0){#5}}
%%%===================================================================================
\def\uput{\@ifnextchar*{\mathuput@i}{\mathuput@i{}}}
\def\mathuput@i#1{\@ifnextchar[{\mathuput@ii{#1}3pt}{\mathuput@ii{#1}}}
\def\mathuput@ii#1#2[{\@ifnextchar({\mathuput@iii{#1}{#2}[}{\mathuput#1{#2}[}}
\def\mathuput@iii#1#2[(#3)]{%
  \vnode(#3){uputangle}
  \mathuput#1{#2}[(!V@uputangle)]}
\def\mathuput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\uput@ii}{\uput@i}}}
%%%===================================================================================
\makeatother
\endinput

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 
